Fast Estimation of Percolation Centrality

In this work, we present a new algorithm to approximate the percolation centrality of every node in a graph. Such a centrality measure quantifies the importance of the vertices in a network during a contagious process. In this paper, we present a randomized approximation algorithm that can compute probabilistically guaranteed high-quality percolation centrality estimates, generalizing techniques used by Pellegrina and Vandin (TKDD 2024) for the betweenness centrality. The estimation obtained by our algorithm is within $\varepsilon$ of the value with probability at least $1-\delta$, for fixed constants $\varepsilon,\delta \in (0,1)$. We our theoretical results with an extensive experimental analysis on several real-world networks and provide empirical evidence that our algorithm improves the current state of the art in speed, and sample size while maintaining high accuracy of the percolation centrality estimates.

==> tables/speedup.tex <==
\begin{table*}[htb!]
\centering
\begin{tabular}{ccccccccccc}
                                            &         & \multicolumn{3}{c}{Speedup}                        &                                         &                                       &         & \multicolumn{3}{c}{Speedup}      \\ \cline{3-5}
\multicolumn{1}{l}{Graph}                   & Epsilon & T(ERA) & T(Fixed) & T(Exact)                       &                                         & \multicolumn{1}{l}{Graph}             & Epsilon & T(ERA)   & T(Fixed) & T(Exact)   \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Musae Fb.}}} & 0.1     & 34.917 & -31.893  & \multicolumn{1}{c|}{6367.360}  & \multicolumn{1}{c|}{\multirow{40}{*}{}} & \multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Web-Not. dame}}}   & 0.1     & -8.358   & -23.142  & 40219.997  \\
                                            & 0.07    & 51.906 & -6.316   & \multicolumn{1}{c|}{4642.547}  & \multicolumn{1}{c|}{}                   &                                       & 0.07    & 40.929   & 32.692   & 34577.321  \\
                                            & 0.05    & 67.094 & 27.977   & \multicolumn{1}{c|}{3219.212}  & \multicolumn{1}{c|}{}                   &                                       & 0.05    & 66.423   & 126.554  & 28367.665  \\
                                            & 0.01    & 94.246 & 800.842  & \multicolumn{1}{c|}{873.655}   & \multicolumn{1}{c|}{}                   &                                       & 0.01    & 92.537   & 1000.329 & 4732.769   \\
                                            & 0.005   & 96.398 & 1510.892 & \multicolumn{1}{c|}{334.734}   & \multicolumn{1}{c|}{}                   &                                       & 0.005   & 96.738   & 2698.100 & 2617.221   \\
\multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Enron}}}           & 0.1     & 29.206 & -23.935  & \multicolumn{1}{c|}{7721.599}  & \multicolumn{1}{c|}{}                   & \multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Web-Google}}}      & 0.1     & 44.686   & 47.271   & 297992.812 \\
                                            & 0.07    & 44.033 & 0.775    & \multicolumn{1}{c|}{5671.016}  & \multicolumn{1}{c|}{}                   &                                       & 0.07    & 62.168   & 146.225  & 249256.027 \\
                                            & 0.05    & 57.934 & 23.588   & \multicolumn{1}{c|}{3616.191}  & \multicolumn{1}{c|}{}                   &                                       & 0.05    & 75.451   & 254.726  & 188000.496 \\
                                            & 0.01    & 93.462 & 828.455  & \multicolumn{1}{c|}{1049.259}  & \multicolumn{1}{c|}{}                   &                                       & 0.01    & 93.885   & 1619.787 & 37490.356  \\
                                            & 0.005   & 96.623 & 1797.223 & \multicolumn{1}{c|}{502.662}   & \multicolumn{1}{c|}{}                   &                                       & 0.005   & 96.881   & 3372.279 & 18878.245  \\
\multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{CA-AstroPH}}}            & 0.1     & 20.548 & -39.632  & \multicolumn{1}{c|}{3343.383}  & \multicolumn{1}{c|}{}                   & \multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Web-Berkstan}}}    & 0.1     & -198.765 & -72.019  & 39513.226  \\
                                            & 0.07    & 30.457 & -19.181  & \multicolumn{1}{c|}{2316.505}  & \multicolumn{1}{c|}{}                   &                                       & 0.07    & -61.718  & -44.851  & 41736.479  \\
                                            & 0.05    & 53.377 & 6.040    & \multicolumn{1}{c|}{1617.267}  & \multicolumn{1}{c|}{}                   &                                       & 0.05    & 6.662    & 3.473    & 40568.762  \\
                                            & 0.01    & 92.916 & 755.129  & \multicolumn{1}{c|}{477.817}   & \multicolumn{1}{c|}{}                   &                                       & 0.01    & 92.075   & 1719.315 & 29943.580  \\
                                            & 0.005   & 95.769 & 1415.967 & \multicolumn{1}{c|}{175.884}   & \multicolumn{1}{c|}{}                   &                                       & 0.005   & 96.491   & 4360.632 & 17521.871  \\
\multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Epinions}}}          & 0.1     & 17.721 & -24.691  & \multicolumn{1}{c|}{16166.030} & \multicolumn{1}{c|}{}                   & \multirow{5}{*}{10\_flickr}           & 0.1     & 57.163   & 160.614  & --         \\
                                            & 0.07    & 43.940 & 25.797   & \multicolumn{1}{c|}{12044.258} & \multicolumn{1}{c|}{}                   &                                       & 0.07    & 66.440   & 203.000  & --         \\
                                            & 0.05    & 60.243 & 52.769   & \multicolumn{1}{c|}{7796.176}  & \multicolumn{1}{c|}{}                   &                                       & 0.05    & 75.054   & 310.836  & --         \\
                                            & 0.01    & 92.651 & 776.115  & \multicolumn{1}{c|}{1773.892}  & \multicolumn{1}{c|}{}                   &                                       & 0.01    & 95.692   & 2465.911 & --         \\
                                            & 0.005   & 96.038 & 1562.221 & \multicolumn{1}{c|}{814.066}   & \multicolumn{1}{c|}{}                   &                                       & 0.005   & 98.067   & 5614.729 & --         \\
\multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Slashdot}}}          & 0.1     & 33.675 & -9.020   & \multicolumn{1}{c|}{23656.103} & \multicolumn{1}{c|}{}                   & \multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Wiki Talks}}}       & 0.1     & 62.475   & 192.934  & --         \\
                                            & 0.07    & 52.709 & 39.302   & \multicolumn{1}{c|}{17923.415} & \multicolumn{1}{c|}{}                   &                                       & 0.07    & 72.238   & 264.312  & --         \\
                                            & 0.05    & 65.907 & 81.187   & \multicolumn{1}{c|}{12330.862} & \multicolumn{1}{c|}{}                   &                                       & 0.05    & 75.763   & 322.113  & --         \\
                                            & 0.01    & 93.601 & 939.131  & \multicolumn{1}{c|}{2959.759}  & \multicolumn{1}{c|}{}                   &                                       & 0.01    & 95.992   & 2662.596 & --         \\
                                            & 0.005   & 96.492 & 1845.325 & \multicolumn{1}{c|}{1387.002}  & \multicolumn{1}{c|}{}                   &                                       & 0.005   & 98.143   & 5853.541 & --         \\
\multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Cit-HepPh}}}             & 0.1     & 8.129  & -36.593  & \multicolumn{1}{c|}{3942.289}  & \multicolumn{1}{c|}{}                   & \multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Twitter}}} & 0.1     & 52.581   & 128.122  & --         \\
                                            & 0.07    & 55.358 & 6.481    & \multicolumn{1}{c|}{4481.463}  & \multicolumn{1}{c|}{}                   &                                       & 0.07    & 67.374   & 215.646  & --         \\
                                            & 0.05    & 65.538 & 79.814   & \multicolumn{1}{c|}{3374.428}  & \multicolumn{1}{c|}{}                   &                                       & 0.05    & 70.542   & 245.556  & --         \\
                                            & 0.01    & 91.578 & 846.856  & \multicolumn{1}{c|}{677.424}   & \multicolumn{1}{c|}{}                   &                                       & 0.01    & 96.012   & 2677.572 & --         \\
                                            & 0.005   & 95.612 & 1937.918 & \multicolumn{1}{c|}{291.363}   & \multicolumn{1}{c|}{}                   &                                       & 0.005   & 98.145   & 5860.559 & --         \\
\multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Twitch-Edges}}}   & 0.1     & 15.361 & -30.922  & \multicolumn{1}{c|}{55613.935} & \multicolumn{1}{c|}{}                   & \multirow{5}{*}{\rotatebox[origin=c]{90}{soc-Pokec}}       & 0.1     & 44.550   & 98.342   & --         \\
                                            & 0.07    & 46.015 & 11.082   & \multicolumn{1}{c|}{51566.034} & \multicolumn{1}{c|}{}                   &                                       & 0.07    & 64.774   & 186.285  & --         \\
                                            & 0.05    & 47.120 & 21.156   & \multicolumn{1}{c|}{30800.224} & \multicolumn{1}{c|}{}                   &                                       & 0.05    & 71.778   & 261.846  & --         \\
                                            & 0.01    & 56.112 & 64.748   & \multicolumn{1}{c|}{1648.988}  & \multicolumn{1}{c|}{}                   &                                       & 0.01    & 95.741   & 2498.553 & --         \\
                                            & 0.005   & 83.772 & 328.227  & \multicolumn{1}{c|}{1047.975}  & \multicolumn{1}{c|}{}                   &                                       & 0.005   & 98.119   & 5778.731 & --         \\
\multirow{5}{*}{\rotatebox[origin=c]{90}{\texttt{Gnutella 31}}}        & 0.1     & 23.025 & -4.832   & \multicolumn{1}{c|}{9961.266}  & \multicolumn{1}{c|}{}                   &                                       &         &          &          &            \\
                                            & 0.07    & 45.630 & 61.792   & \multicolumn{1}{c|}{8121.749}  & \multicolumn{1}{c|}{}                   &                                       &         &          &          &            \\
                                            & 0.05    & 66.415 & 89.468   & \multicolumn{1}{c|}{5527.188}  & \multicolumn{1}{c|}{}                   &                                       &         &          &          &            \\
                                            & 0.01    & 91.766 & 852.688  & \multicolumn{1}{c|}{1110.996}  & \multicolumn{1}{c|}{}                   &                                       &         &          &          &            \\
                                            & 0.005   & 95.875 & 1846.266 & \multicolumn{1}{c|}{536.601}   & \multicolumn{1}{c|}{}                   &                                       &         &          &          &            \\ \hline
\end{tabular}
\end{table*}

==> trunk/related_works.tex <==
\section{Related Works}

